A Lightweight Image Super-Resolution Transformer Trained on Low-Resolution Images Only

Transformer architectures prominently lead single-image super-resolution (SISR) benchmarks, reconstructing high-resolution (HR) images from their low-resolution (LR) counterparts. Their strong representative power, however, comes with a higher demand for training data compared to convolutional neural networks (CNNs). For many real-world SR applications, the availability of high-quality HR training images is not given, sparking interest in LR-only training methods. The LR-only SISR benchmark mimics this condition by allowing only low-resolution (LR) images for model training. For a 4x super-resolution, this effectively reduces the amount of available training data to 6.25% of the HR image pixels, which puts the employment of a data-hungry transformer model into question. In this work, we are the first to utilize a lightweight vision transformer model with LR-only training methods addressing the unsupervised SISR LR-only benchmark. We adopt and configure a recent LR-only training method from microscopy image super-resolution to macroscopic real-world data, resulting in our multi-scale training method for bicubic degradation (MSTbic). Furthermore, we compare it with reference methods and prove its effectiveness both for a transformer and a CNN model. We evaluate on the classic SR benchmark datasets Set5, Set14, BSD100, Urban100, and Manga109, and show superior performance over state-of-the-art (so far: CNN-based) LR-only SISR methods. The code is available on GitHub: https://github.com/ifnspaml/SuperResolutionMultiscaleTraining.

==> figures/latex_embedding/fig_method.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.77\textwidth]{figures/method.png}
\caption{{\bf Training data preprocessing} for our proposed MST++ method.}
\vspace*{-2mm}
\label{fig:method}
\end{figure*}

==> figures/quali_comp/urban100_030_v4_subfigure.tex <==
%\begin{figure*}[htbp]
%\captionsetup[subfigure]{justification=centering} %to center the captions that span two lines
    \centering
    % Original Image
    \raisebox{0.0\height}{
    \begin{subfigure}[b]{0.205\textwidth}
        \centering
        %\raisebox{2cm}{
        %\vspace{-4.7cm}
        \vfill
        \includegraphics[width=0.74\textwidth]{figures/quali_comp/urban100_030/img_030.png}
        %\captionsetup{skip=1cm} % adjust the space between image and caption
        %}
        \vfill
        \caption*{Urban100 img\_030}
        \label{fig:original}
    \end{subfigure}%
    }
    \hfill
    %\hspace{0.005\textwidth}
    \begin{subfigure}[b]{0.74\textwidth}
        \centering
        % Top row
        \begin{subfigure}[b]{0.16\textwidth}
        \hspace{-2mm}
            \centering
            \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/lr_roi.png}
            \caption*{LR \\ \phantom{}}
        \end{subfigure}%
        %\hspace{-1mm}
        \begin{subfigure}[b]{0.16\textwidth}
         \hspace{1.5mm}
            \centering
            \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/reference_roi.png}
            \caption*{GT \\ (PSNR / SSIM)}
        \end{subfigure}%
        \hspace{0.01\textwidth}
        \begin{subfigure}[b]{0.32\textwidth}
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/SimUSR.png}
                %\caption*{}
            \end{subfigure}%
             \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/SimUSR_delta_map.png}
                %\caption*{}
            \end{subfigure}%
            \caption*{SimUSR + \texttt{CARN} \\ (0.00 / 0.0000)}
        \end{subfigure}%
        \hspace{0.01\textwidth}
        \begin{subfigure}[b]{0.32\textwidth}
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/MSTbic.png}
                %\caption*{MSTbic}
            \end{subfigure}%
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/MSTbic_delta_map.png}
                %\caption*{}
            \end{subfigure}%
            \caption*{MSTbic+\texttt{CARN} \\ (0.00 / 0.0000)}
        \end{subfigure}%
        \hfill
        % Bottom row
        \begin{subfigure}[b]{0.32\textwidth}
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/bicubic.png}
                %\caption*{}
            \end{subfigure}%
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/bicubic_delta_map.png}
                %\caption*{Bicubic delta}
            \end{subfigure}%
            \caption*{Bicubic \\ (17.43 / 0.5813)}
        \end{subfigure}%
        \hspace{0.01\textwidth}
        \begin{subfigure}[b]{0.32\textwidth}
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/SimUSR.png}
                %\caption*{SimUSR SwinIR lw}
            \end{subfigure}%
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/SimUSR_delta_map.png}
                %\caption*{SimUSR delta}
            \end{subfigure}%
            \caption*{SimUSR + \texttt{SwinIR lw}\\(20.84 / 0.8864)}
        \end{subfigure}%
        \hspace{0.01\textwidth}
        \begin{subfigure}[b]{0.32\textwidth}
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/MSTbic.png}
                %\caption*{MSTbic}
            \end{subfigure}%
            \begin{subfigure}[b]{0.5\textwidth}
                \centering
                \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/MSTbic_delta_map.png}
                %\caption*{MSTbic}
            \end{subfigure}%
        \caption*{MSTbic + \texttt{SwinIR lw} \\ (23.93 / 0.9259)}
        \end{subfigure}%
        %\vspace{-0.5em} % Adjust this value to reduce the space between the rows if necessary   
    \end{subfigure}
    \raisebox{0.06\height}{
    \begin{subfigure}[b]{0.03\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/quali_comp/urban100_04/scale_bar.png}
        \label{fig:scale_bar}
     \end{subfigure}
    }
    %\hfill
%\end{figure*}
